OPITeR: A program for tensor reduction of multi-loop Feynman Integrals

We present OPITeR, a FORM program for the reduction of multi-loop tensor Feynman integrals. The program can handle tensors, including spinor indices, with rank of up to 20 and can deal with up to 8 independent external momenta. The reduction occurs in $D$ dimensions compatible with conventional dimensional regularization. The program is able to manifest symmetries of the integrand in the tensor reduced form.

==> algorithms.tex <==
In this section we shall describe some of the more novel algorithms employed in the \OPITER{} program.

\subsubsection{Basis Transformations}
The first basis transformation we perform is transforming into the antisymmetric basis of gamma matrices. We do this as it has nice orthogonality properties we can exploit when taking traces \cite{Kennedy:1981kp}.  The antisymmetric gamma matrices are defined as 

\begin{equation}\label{eq:antisymmetric-gamma}
    \Gamma^{\mu_1\dots\mu_p}=\gamma^{[\mu_1}\dots\gamma^{\mu_p]}= \frac{1}{p!}\,\delta^{\mu_1\dots\mu_p}_{\nu_1\dots\nu_p}\gamma^{\nu_1}\dots\gamma^{\nu_p}\,.
\end{equation}
There is an efficient way to convert from a product of gamma matrices to an antisymmetric $\Gamma$
\begin{equation}
    \label{eq:gammatoGamma}
    \gamma^{\mu_1}\dots\gamma^{\mu_n}=\sum_{k=0}^{n}\sum_{\pi\in \Sigma_n^k}\sgn(\pi)\Gamma^{\mu_{\pi{(1)}}\dots\mu_{\pi(k)}}\tr(\gamma^{\mu_{\pi(k+1)}}\dots\gamma^{\mu_{\pi(n)}})\,,
\end{equation}
    where the sum over $\Sigma_{n}^k$ shuffles the first $k$ indices with the remaining $n-k$ indices over the two tensors. This is very simple to implement in \FORM. The indices of the product of gamma matrices on the left are split between the $\Gamma$ and trace then permuted with the appropriate sign using the \FORM's \verb|distrib_| function. The trace is then done with \FORM's built in implementation of gamma matrices. This occures when the procedure \verb|gamma2Gamma| is called. 

    The transformation into the Van Neerven-Vermaseren basis is performed as part of the tensor reduction stage. In \verb|tenred| and \verb|tenredisym| Loop momenta are decomposed by applying \cref{eq:loopdecomp}. The sum is performed by making a copy of the \verb|ext| function
    then iteratively removing an element from a list and then adding to the expansion the appropriate momenta multiplied by the inverse Gram element. After the reduction the transformation out this basis in performed by two procedures: \verb|expanddt| and \verb|dual2ext|. To transform the transverse metric we apply
    \begin{align}
        g_\perp^{\mu\nu} &=  g^{\mu\nu} -\sum_{i,j=1}^E  q_i{}^\mu\, H_{ij}\,  q_j{}^\nu\,,\\
        {p_i}_\perp\cdot{p_j}_\perp &= {p_i}\cdot{p_j} -\sum_{l,m=1}^E  p_i\cdot q_l\, H_{lm}\,  q_m\cdot p_j\,.
    \end{align} 
    The sums are performed by making two copies of the \verb|ext| function and then iterating over both of them as above. The transformation of the dual momenta $r_i$ is done by applying \cref{eq:momentumtransform} and performing the sum as above.
    

\subsubsection{Tensor reduction}

The most general tensor reduction occurs in the procedure \verb|tenred|. It proceeds by:
\begin{itemize}
    \item Loop momenta are decomposed into the Van Neerven-Vermaseren basis.
    \item The loop momenta with Lorentz indices are extracted.
    \item The indices are used to generate all possible elements of the basis through  \verb|dd_|.
    \item A copy of each tensor is stored and the individual metrics are combined into projectors  contracted with the loop momenta by \verb|PrtCanonicalize|.
\end{itemize}

\subsubsection{Tensor reduction with integrand symmetry}

To begin determining the  integrand symmetry decomposition we relabel all the user provided loop momenta $p_i \rightarrow$ \verb|qqi| a function \verb|FF2| stores the index and momenta correspondence. We move the vector to the argument
\begin{itemize}
    \item  Loop momenta are decomposed into the Van Neerven-Vermaseren basis.
    \item  The loop momenta with Lorentz indices are relabeled  $p_i \rightarrow$ \verb|qqi|, and extracted. The correspondence between momenta and its index is stored. 
    \item All possible monomials $m(\alpha)$ and combinatorial factors $c(\alpha)$ are generated using by contracting all the momenta with \verb|dd_| (see \cref{eq:dperpcontracted}).
    \item Each dot product of momenta is copied, on one of them the substitution \verb|qqi| $\rightarrow$ \verb|ppi| is made. These are combined into contracted projectors by \verb|PrtCanonicalize|. 
    \item The symmetry of the integrand is extracted by collecting all the indices which had the same momenta. This forms the symmetriser.  
    \item A single term that will generate the $T(\alpha)$ when acted on by the symmetriser is created by taking a monomial in the \verb|qqi| momenta. A dot product is replaced by a metric \verb|qqi.qqj| $\rightarrow$ \verb|ddt(qqi,qqj)| and then the momenta is replaced with one of the indices that momenta had originally.
\end{itemize}
\begin{equation}
T^{\mu_1\dots\mu_N}(\alpha) = (\mathcal{S}_{N_1,\dots,N_L})^{\mu_1\dots\mu_N}_{\nu_1\dots\nu_N}t^{\nu_1\dots\nu_N}(\alpha)
\end{equation}
\begin{equation}
    \begin{split}
    (\mathcal{S}_{N_1,\dots,N_L})^{\mu_1\dots\mu_N}_{\nu_1\dots\nu_N}=& \sum_{\sigma_1\in S_{N_1}}\delta^{\mu_1}_{\nu_{1,\sigma_1(1)}}\dots \delta^{\mu_{N_1}}_{\nu_{1,\sigma_1(N_1)}}\times\\\times& \sum_{\sigma_2\in S_{N_2}}\delta^{\mu_{N_1+1}}_{\nu_{2,\sigma_2(1)}}\dots \delta^{\mu_{N_1+N_2}}_{\nu_{2,\sigma_2(N_2)}}\times  \\
    &\dots \\
     \times& \sum_{\sigma_L\in S_{N_L}}\delta^{N-N_l}_{L,\nu_{\sigma_L(1)}}\dots \delta^{\mu_{N}}_{\nu_{L,\sigma_L(N_L)}}
    \end{split}
\end{equation}
\subsubsection{Canonicalizing the projectors}
The procedure \verb|PrtCanonicalize| simply takes a projector from one of the reduction procedures and formats it in terms of the tables that store the contracted projectors. If it's contractions have not been calculated it applies the most general version of the projector.
